Domain wall QCD with physical quark masses

We present results for several light hadronic quantities ($f_\pi$, $f_K$, $B_K$, $m_{ud}$, $m_s$, $t_0^{1/2}$, $w_0$) obtained from simulations of 2+1 flavor domain wall lattice QCD with large physical volumes and nearly-physical pion masses at two lattice spacings. We perform a short, O(3)%, extrapolation in pion mass to the physical values by combining our new data in a simultaneous chiral/continuum `global fit' with a number of other ensembles with heavier pion masses. We use the physical values of $m_\pi$, $m_K$ and $m_\Omega$ to determine the two quark masses and the scale - all other quantities are outputs from our simulations. We obtain results with sub-percent statistical errors and negligible chiral and finite-volume systematics for these light hadronic quantities, including: $f_\pi$ = 130.2(9) MeV; $f_K$ = 155.5(8) MeV; the average up/down quark mass and strange quark mass in the $\bar {\rm MS}$ scheme at 3 GeV, 2.997(49) and 81.64(1.17) MeV respectively; and the neutral kaon mixing parameter, $B_K$, in the RGI scheme, 0.750(15) and the $\bar{\rm MS}$ scheme at 3 GeV, 0.530(11).

==> text_sections/BKtabs.tex <==
$48^3 \gamma$:
% a^-1=1.7294
%mom: 8tw1 9 9tw0.5 9tw1 10
\begin{center}
\begin{tabular}{c|ccccc}
\hline
$q$/GeV & 2.72125 & 2.88132 & 2.96136 & 3.04139 & 3.20147 \\
\hline
VV+AA & 1.20472(14) & 1.21216(8) & 1.21604(8) & 1.21996(8) & 1.22827(6) \\
V & 1.05201(5) & 1.05371(3) & 1.05463(4) & 1.05557(3) & 1.05753(1) \\
A & 1.05196(3) & 1.05368(2) & 1.05458(4) & 1.05553(3) & 1.05745(4) \\
\end{tabular}
\end{center}
3eV : Extrapolate: 0.913967 + 3.40488e-05 - 2.13359e-05
3GeV 1sigma away : Extrapolate: 0.914069 + 3.82191e-05 - 2.28748e-05

$48^3 \slashed q$:
% a^-1=1.7294
%mom: 8tw1 9 9tw0.5 9tw1 10
\begin{center}
\begin{tabular}{c|ccccc}
\hline
$q$/GeV & 2.72125 & 2.88132 & 2.96136 & 3.04139 & 3.20147 \\
\hline
VV+AA & 1.29658(31) & 1.30250(14) & 1.30598(10) & 1.30955(10) & 1.31773(25) \\
V & 1.11640(15) & 1.11660(7) & 1.11697(4) & 1.11749(5) & 1.11902(15) \\
A & 1.11633(13) & 1.11659(5) & 1.11695(4) & 1.11747(5) & 1.11902(14) \\
\end{tabular}
\end{center}
3GeV : Extrapolate: 0.954452 + 3.87901e-05 - 3.14675e-05
3GeV 1sigma away : Extrapolate: 0.95459 + 4.15712e-05 - 3.25182e-05


$64^3 \gamma q$:
% a^-1=2.3576
%mom: 8tw1 9 9tw0.5 9tw1 10
\begin{center}
\begin{tabular}{c|ccccc}
\hline
$q$/GeV & 2.7823 & 2.94596 & 3.0278 & 3.10963 & 3.27329 \\
\hline
VV+AA & 1.13936(9) & 1.14363(10) & 1.14575(6) & 1.14798(6) & 1.15261(4) \\
V & 1.03721(4) & 1.03783(3) & 1.03818(2) & 1.03859(2) & 1.03949(2) \\
A & 1.03715(2) & 1.03780(3) & 1.03815(2) & 1.03856(2) & 1.03949(1) \\
\end{tabular}
\end{center}
3GeV : Extrapolate: 0.941055 + 1.90793e-05 - 1.717e-05
3GeV 1sigma away : Extrapolate: 0.94117 + 1.94401e-05 - 1.94418e-05

$64^3 \slashed q$:
% a^-1=2.3576
%mom: 8tw1 9 9tw0.5 9tw1 10
\begin{center}
\begin{tabular}{c|ccccc}
\hline
$q$/GeV & 2.7823 & 2.94596 & 3.0278 & 3.10963 & 3.27329 \\
\hline
VV+AA & 1.22136(20) & 1.22299(22) & 1.22387(12) & 1.22501(11) & 1.22760(12) \\
V & 1.09622(9) & 1.09451(11) & 1.09379(6) & 1.09323(5) & 1.09239(6) \\
A & 1.09619(9) & 1.09449(11) & 1.09377(6) & 1.09321(5) & 1.09238(7) \\
\end{tabular}
\end{center}
3GeV : Extrapolate: 0.978152 + 2.24154e-05 - 1.95451e-05
3GeV 1sigma away : Extrapolate: 0.978346 + 2.27631e-05 - 2.04446e-05

$32fine^3 \gamma$:
% a^-1=3.145
%mom: 2tw1 3 3tw1 4 4tw1 5
\begin{center}
\begin{tabular}{c|cccccc}
\hline
$q$/GeV & 2.18326 & 2.61991  & 3.05656  & 3.49322  & 3.92987 & 4.36652  \\
\hline
VV+AA & 1.08793(30) & 1.09602(53) & 1.10356(30) & 1.11137(28) & 1.11909(12) & 1.12751(11) \\
V & 1.03160(12) & 1.03005(15) & 1.02984(8) & 1.03049(8) & 1.03162(5) & 1.03327(4) \\
A & 1.03076(11) & 1.02976(17) & 1.02972(8) & 1.03042(8) & 1.03159(5) & 1.03324(5) \\
\end{tabular}
\end{center}
3GeV : Extrapolate: 0.961695 + 0.00014261 - 0.000120587
3GeV 1sigma away : Extrapolate: 0.961962 + 0.000135137 - 0.000124635

$32fine^3 \slashed q$:
% a^-1=3.145
%mom: 2tw1 3 3tw1 4 4tw1 5
\begin{center}
\begin{tabular}{c|cccccc}
\hline
$q$/GeV & 2.18326 & 2.61991  & 3.05656  & 3.49322  & 3.92987 & 4.36652  \\
\hline
VV+AA & 1.18143(36) & 1.17928(112) & 1.17863(65) & 1.18050(63) & 1.18350(28) & 1.18855(25) \\
V & 1.10353(55) & 1.09220(57) & 1.08465(34) & 1.08013(31) & 1.07727(14) & 1.07605(12) \\
A & 1.10308(55) & 1.09196(57) & 1.08453(34) & 1.08005(31) & 1.07723(14) & 1.07601(12) \\
\end{tabular}
\end{center}
3GeV : Extrapolate: 0.999467 + 0.000120753 - 7.6339e-05
3GeV 1sigma away : Extrapolate: 0.999975 + 0.000119353 - 7.6337e-05





